Analysis of Unconstrained Nonlinear MPC Schemes with Time Varying Control Horizons

For nonlinear discrete time systems satisfying a controllability condition, we present a stability condition for model predictive control without stabilizing terminal constraints or costs. The condition is given in terms of an analytical formula which can be employed in order to determine a prediction horizon length for which asymptotic stability or a performance guarantee is ensured. Based on this formula a sensitivity analysis with respect to the prediction and the possibly time varying control horizon is carried out.

==> recap.tex <==
\section{RECAP}\label{recap}


\juergen{Ich wuerde hier mit dem Stabilitaetsresultat anfangen:
\cite{GR2008} \cite{LR2006}
\begin{theorem} \label{TheoremStabilityTimeVaryingControlHorizon}
	Suppose a multistep feedback law $\feedback_{N, m^\star}: \stateset \times \{ 0, \ldots, m^\star - 1\} \to \controlset$, a set $\controlset \subseteq \{ 1, \ldots, m^\star\}$ and a function $V_N: \stateset \to \R_0^+$ are given. If for all control horizon sequence $(m_k)_{k \in \N_0}$ with $m_k \in \controlset$ for all $k \in \N_0$ and for each $\state \in \stateset$ we have
	\begin{align}
		\label{NotationRelaxedLyapunovInequality}
		& V(\state(\updateinstant(k)) - V(\state(\updateinstant(k+1)) \nonumber \\
		& \geq \alpha \sum_{i = 0}^{m_k} \stagecost \left( \state(\updateinstant(k)+i), \feedback_{N, m^\star}( \state( \updateinstant(k)+i, i ) ) \right)
	\end{align}
	for some $\alpha\in(0,1]$ and all $k \in \N_0$, then the estimate $\alpha V_\infty(\state) \leq \alpha V_\infty^{\feedback_{N,m^\star}}(\state) \leq V_N(\state)$ holds for all $\state \in \stateset$ and all $(m_k)_{k \in \N_0}$ with $m_k \in \controlset$.
\end{theorem}
Danach laesst sich denke ich gut motivieren, warum wir $\alpha$ gerne fuer alle $N$ und $m$ bestimmt haetten.
Dazu dann die controllability assumption
\begin{assumption}\label{AssumptionControllabilityCondition}
	Given a function $\beta \in \KLzero$, for each $\statezero \in X$ there exists a control function $\control_{\statezero} \in \admissiblecontrolset^\infty$ satisfying $\stagecost(\state_{\control_{\statezero}}(n), \control_{\statezero}(n)) \leq \beta(\stagecoststar(\statezero), n)$ for all $n \in \N_0$.
\end{assumption}
Hieraus wuerde ich im Fliesstext die Bedingungen fuer das Minimierungsproblem 
\begin{align}
	\label{MinimierungsproblemSchranke1}
	\sum_{n = k}^{N-1} \stageabbreviation_n \leq \boundabbreviation_{N-k}(\stageabbreviation_k), \quad k = 0, \ldots, N-2
\end{align}
\begin{align}
	\label{MinimierungsproblemSchranke2}
	\valuefunctionabbreviation \leq \sum_{n = 0}^{j-1} \stageabbreviation_{n+m} + \boundabbreviation_{N-j}(\stageabbreviation_{j+m}), \quad j = 0, \ldots, N-m-1
\end{align}
einfuehren und sagen, dass falls zusaetzlich
\begin{align}
	\label{BedingungStabilitaet}
	\sum_{n=0}^{N-1} \stageabbreviation_n - \valuefunctionabbreviation \geq \alpha \sum_{n=0}^{m-1} \stageabbreviation_n \quad \text{for some $\alpha \in (0, 1]$}
\end{align}
gilt, dass wir dann Stabilitaet und die Abschaetzung aus Theorem \ref{TheoremStabilityTimeVaryingControlHorizon} erhalten.
Dann kaeme das Minimierungsproblem
\begin{quote}
	For a given $\beta \in \KLzero$, optimization horizon $N \geq 1$ and control horizon $m \in \{1, \ldots, N - 1\}$ we compute the upper bound of infima $\alpha$ from \eqref{BedingungStabilitaet} with respect to $\stageabbreviation_0$, \ldots, $\stageabbreviation_{N-1}$ and $\valuefunctionabbreviation$
	\begin{align*}
		\alpha := \inf_{\stageabbreviation_0, \ldots, \stageabbreviation_{N-1}, \valuefunctionabbreviation} \frac{\sum_{n=0}^{N-1} \stageabbreviation_n - \valuefunctionabbreviation}{\sum_{n=0}^{m-1} \stageabbreviation_n}
	\end{align*}
	subject to the constraints \eqref{MinimierungsproblemSchranke1}, \eqref{MinimierungsproblemSchranke2} and $\stageabbreviation_0$, \ldots, $\stageabbreviation_{N-1}$, $\valuefunctionabbreviation > 0$.
\end{quote}}


\vspace*{1cm}
\karl{ich wuerde gleich Linearitaet von $\beta(r,t)$ in $r$ voraussetzen und sowohl die Kontrollierbarkeitsannahme als auch alles Weitere so aufschreiben. Zudem ein Verweis, falls diese Linearitaet nicht gegeben ist.}

\karl{wann soll der Nachweis der asymptotischen Stabilitaet fuer zeitvarianten Kontrollhorizont erfolgen? Dies war ein neues Resultat, wenn auch kein besonderes Spannendes vom mathematischen Standpunkt aus;-)}

